Clock Distribution with Gradient TRIX

Gradient clock synchronization (GCS) algorithms minimize the worst-case clock offset between the nodes in a distributed network of diameter $D$ and size $n$. They achieve optimal offsets of $\Theta(\log D)$ locally, i.e. between adjacent nodes as shown by Lenzen et al., and $\Theta(D)$ globally as shown by Biaz and Welch. As demonstrated in the work of Bund et al., this is a highly promising approach for improved clocking schemes for large-scale synchronous Systems-on-Chip (SoC). Unfortunately, in large systems, faults hinder their practical use. State of the art fault-tolerant, as presented by Bund et al., has a drawback that is fatal in this setting: It relies on node and edge replication. For $f=1$, this translates to at least $16$-fold edge replication and high degree nodes, far from the optimum of $2f+1=3$ for tolerating up to $f$ faulty neighbors. In this work, we present a self-stabilizing GCS algorithm for a grid-like directed graph with optimal node in- and out-degrees of $3$ that tolerates $1$ faulty in-neighbor. If nodes fail with independent probability $p\in o(n^{-1/2})$, it achieves asymptotically optimal local skew of $\Theta(\log D)$ with probability $1-o(1)$; this holds under general worst-case assumptions on link delay and clock speed variations, provided they change slowly relative to the speed of the system. The failure probability is the largest possible ensuring that with probabity $1-o(1)$ for each node at most one in-neighbor fails. As modern hardware is clocked at gigahertz speeds and the algorithm can simultaneously sustain a constant number of arbitrary changes due to faults in each clock cycle, this results in sufficient robustness to dramatically increase the size of reliable synchronously clocked SoCs.

==> app_modelling.tex <==
\section{Motivating our Model: An Exercise in Theory Building}\label{sec:app_motivation}
In this final section, we take a closer look at some of our modelling choices that might appear strange at first glance. A key motivation of this work is to produce theoretically correct algorithms which can be applied to the synchronous clocking of VLSI systems. This guides our modelling choices on two fronts:
\begin{itemize}
    \item \textbf{Our Topology}: At a very high level, we would like to synchronise so-called clock islands on modern VLSI systems that currently rely on expensive asynchronous communication. This naturally suggests a grid-like topology. However, a simple grid does not suffice. Even with our extremely sparse network connectivity, we require each node in every row to have three neighbours in adjacent rows, meaning that the nodes at the right and left boundary ``miss'' a neighbor.
    Mathematically, the most elegant solution would be a cylinder, but embedding it on a rectangular grid induces a wasteful factor~2 overhead.
    Instead, we fall back to replicating each node on the right and left boundary once and connecting the two copies. Our scheme is phrased in a more general way, allowing for arbitrary base graphs of minimum degree 2. Our approach achieves this at asymptotically negligible overhead.
    \item \textbf{Our Fault Model}: Here, we strike a fine balance between practical viability and the theoretical optimum. A large class of permanent faults can be chalked up to manufacturing process variations and aging. While there are correlations, the dominant contributing factors are approximately i.i.d. Further variations due to long voltage droops and temperature variations happen over times ranging a few microseconds \cite{harris2010cmos}; orders of magnitude longer than the typical clock cycle. This justifies assuming that most delays do not change dramatically between consecutive pulses. Note that local oscillators are, ultimately, timed by such delays, so this applies to changes in hardware clock speeds as well. 
\end{itemize}
\vfill
